Rate-capability of the VMM3a Front End in the RD51 Scalable Readout System

The VMM3a is an Application Specific Integrated Circuit (ASIC), specifically developed for the readout of gaseous detectors. Originally developed within the ATLAS New Small Wheel (NSW) upgrade, it has been successfully integrated into the Scalable Readout System (SRS) of the RD51 collaboration. This allows, to use the VMM3a also in small laboratory set-ups and mid-scale experiments, which make use of Micro-Pattern Gaseous Detectors (MPGDs). As part of the integration of the VMM3a into the SRS, the readout and data transfer scheme was optimised to reach a high rate-capability of the entire readout system and profit from the VMM3a's high single-channel rate-capability of 3.6 Mhits/s. The optimisation focused mainly on the handling of the data output stream of the VMM3a, but also on the development of a trigger-logic between the front-end cards and the DAQ computer. In this article, two firmware implementations of the non-ATLAS continuous readout mode are presented, as well as the implementation of the trigger-logic. Afterwards, a short overview on X-ray imaging results is presented, to illustrate the high rate-capability rom an application point-of-view.

==> original-table.tex <==
\begin{table*}[t]
	\centering
	\begin{tabular}{cc|cccccc}
		\toprule
		\multicolumn{2}{c|}{Readout stage} &
		\multicolumn{2}{c}{\multirow{2}{*}{Theoretical limit}} &
		\multicolumn{4}{c}{Measured rate}\\
		\multicolumn{2}{c|}{\textit{Unit Quantity}} & & & \multicolumn{2}{c}{\textit{Before}} & \multicolumn{2}{c}{\textit{After}}\\
		\midrule
		\multirow{2}{*}{\textbf{(A)}} & VMM3a channel & 
		\multirow{2}{*}{\SI{4}{MHz}} & \multirow{2}{*}{\SI{152}{Mbps}} &
		\multirow{2}{*}{\SI{1.8}{MHz}} & \multirow{2}{*}{\SI{68.4}{Mbps}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} \\
		& \textit{Rate per channel} &   &   &   &   &   &  \\
		\multirow{2}{*}{\textbf{(B)}} & VMM3a to Spartan-6 &
		\multirow{2}{*}{\SI{20}{MHz}} & \multirow{2}{*}{\SI{800}{Mbps}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} \\
		& \textit{Rate per VMM3a} &   &   &   &   &   &  \\
		\multirow{2}{*}{\textbf{(C)}} & Spartan-6 &
		\multirow{2}{*}{\SI{8}{MHz}} & \multirow{2}{*}{\SI{320}{Mbps}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} \\
		& \textit{Rate per HDMI-SerDes} &   &   &   &   &   &  \\
		\multirow{2}{*}{\textbf{(D)}} & HDMI & 
		\multirow{2}{*}{\SI{16}{MHz}} & \multirow{2}{*}{\SI{640}{Mbps}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} \\
		& \textit{Rate per Hybrid} &   &   &   &   &   &  \\
		\multirow{2}{*}{\textbf{(E)}} & DVMM and FEC & 
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} \\
		& \textit{Rate per DVMM card} &   &   &   &   &   &  \\
		\multirow{2}{*}{\textbf{(F)}} & Gigabit Ethernet & 
		\multirow{2}{*}{\SI{20.8}{MHz}} & \multirow{2}{*}{\SI{1.0}{Gbps}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} \\
		& \textit{Rate per FEC} &   &   &   &   &   &  \\
		\multirow{2}{*}{\textbf{(G)}} & DAQ computer & 
		\multirow{2}{*}{\SI{20.8}{MHz}} & \multirow{2}{*}{\SI{1.0}{Gbps}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} &
		\multirow{2}{*}{\textbf{\SI{0}{MHz}}} & \multirow{2}{*}{\textbf{\SI{0}{Mbps}}} \\
		& \textit{Rate per Network Port} &   &   &   &   &   &  \\
		\bottomrule
	\end{tabular}
	\caption{Rate-capability of the various stages of VMM3a/SRS, with the
		theoretical maximally possible data rate according to data sheet
		specifications, the measured data rate before performing the
		improvements and the data rate achieved after implementing the
		firmware improvements. \textbf{EVERYTHING THAT IS BOLD NEEDS TO BE UPDATED}}
	\label{tab:results-vs-expectation}
\end{table*}
